Flatness and Complexity of Immediate Observation Petri Nets

In a previous paper we introduced immediate observation (IO) Petri nets, a class of interest in the study of population protocols and enzymatic chemical networks. In the first part of this paper we show that IO nets are globally flat, and so their safety properties can be checked by efficient symbolic model checking tools using acceleration techniques, like FAST. In the second part we study Branching IO nets (BIO nets), whose transitions can create tokens. BIO nets extend both IO nets and communication-free nets, also called BPP nets, a widely studied class. We show that, while BIO nets are no longer globally flat, and their sets of reachable markings may be non-semilinear, they are still locally flat. As a consequence, the coverability and reachability problem for BIO nets, and even a certain set-parameterized version of them, are in PSPACE. This makes BIO nets the first natural net class with non-semilinear reachability relation for which the reachability problem is provably simpler than for general Petri nets.

==> complexity-BIO.tex <==
%!TEX root = main.tex
In~\cite{conf/apn/EsparzaRW19} we prove that the reachability and coverability problems are $\PSPACE$-complete. 
These results also hold for \bio{} nets.

\begin{restatable}{theorem}{TheoremBioReach}
The reachability and coverability problem for \bioLong{} nets are \PSPACE-complete.
\end{restatable}
%
\begin{proof}[Sketch]
IO nets are a subclass of \bio{} nets, so the parameterized problems stay \PSPACE-hard for \bio{} nets. 
By Savitch's Theorem, \NPSPACE=\PSPACE, so it is sufficient to provide a nondeterministic algorithm to prove that these problems are in \PSPACE{}.
We give an idea of the algorithm for reachability from $M'$ to $M$.
The proof of its correctness as well as the algorithm for coverability can be found in the appendix.

Let $m$ the size of $M$.
The intuition for the algorithm is that, if there exists a firing sequence from $M'$ to $M$, then by the Replacement Lemma there exists a fuel-efficient decorated history from $M'$ to $M$.
We guess, step by step, combinations $D_i=C+F+S$ where $C$ (for cargo) is a multiset of $\le m$ elements of $P$, $F$ (for fuel) is a multiset of $\le n^2$ elements of $P$ with at most $n$ elements of the same place, and $S$ (for smoke) is a set/support of places.
%The steps have to verify that there exists a transition $t$ and a iteration $l$ such that “$D_i$ with some number of tokens in $S_i$” reaches “$D_{i+1}$ with some number of tokens in $S_{i+1}$” by firing $t^l$.
The intuition is that, because of the "smoke-irrelevance" Lemma, the number of smoke nodes in the decorated history does not matter.

We start at $D_0=C+F+S$ such that for all $p\in P$, if $M'(p) > m+n$ then $p \in S$, and $C+F(p) =M'(p)$, and if $p \notin S$, then $C+F(p) =M'(p)$. 
The intuition is that, in a fuel-efficient decorated history, if a place contains more than $m+n$ nodes then it must contain at least one smoke node.
We keep guessing until we reach $D=C+F+S$ such that $S=F=\emptyset \land C= L$.
%The problem of coverability can be reduced to the reachability problem by adding "destroying transitions" $\tau_p$
%with preset $\preset{t}=\set{p}$ and postset $\postset{t}=\emptyset$ for every place $p$.
%Details can be found in the appendix
\end{proof}

\cwk{here could be a good place for the remark that these results hold also for multi-observation extensions of the models + no source place in BIO extension}

==> complexity.tex <==
%!TEX root = main.tex
In~\cite{conf/apn/EsparzaRW19} we prove that parameterized versions of the reachability, coverability and liveness problems are $\PSPACE$-complete. 
We recall these results here, and then show that they also hold for \bio{} nets
using the Shortening Theorem.
We recall some definitions of \cite{conf/apn/EsparzaRW19}.

\subparagraph*{Cubes and Counting Constraints}
%%%%copied from PN20 submission
Let $\net=(P,T,F)$ be a Petri net.
A set $\cube$ of markings is a \emph{cube} if there exist mappings $L \colon P \rightarrow \N$ and $U \colon P \rightarrow \N \cup \infty$ such that $M \in \cube$ if and only if $L\leq M \leq U$.
The mappings $L$ and $U$ are the \emph{upper bound} and \emph{lower bound} of $\cube$ respectively, and $(L,U)$ is the \emph{representation} of $\cube$.
The cube represented by $(L,U)$ is denoted $\sem{L,U}$. A \emph{counting constraint} $\cC$ is a finite set  $\set{(L_1,U_1),\ldots, (L_k,U_k)}$ of representations of cubes. A
counting constraint $\cC$ \emph{represents} the set $\sem{\cC} \defeq (L_1,U_1) \cup \ldots \cup (L_k,U_k)$. Sets of markings represented by counting constraints are called \emph{counting sets}.

Notice that a cube has a unique representation; we allow ourselves to use $\cube$ for both the counting set  and the counting constraint.
%However there can be more than one counting constraint for one counting  set.
%For example $\set{(1,3),(2,4)}$ and  $\set{(1,4)}$ define the same counting set, the cube $\sem{1,4}$.
\cwk{there was a definition of cube-norms here, but since there is also one below I commented it out}
%%\subparagraph*{Measures of counting constraints.}
%The $l$-norm and the $u$-norm of a cube $\cube=(L,U)$ are defined by:
%$$\begin{array}{lcl}
%\lnorm{\cube} \defeq \displaystyle \sum_{p \in P} L(p) & \quad & \unorm{\cube} \defeq \displaystyle \sum_{\substack{p\in P\\ U(p)<\infty}} \!\!\!\!U(p) \mbox{ (and \( 0\) if \(U(p)=\infty\) for all \(p\))}.
%\end{array}$$
%The $l$-norm (respectively $u$-norm) of a counting constraint $\cC = \sem{\cube_1,\ldots,\cube_k}$ is the maximum $l$-norm (respectively $u$-norm) of a cube in $\cC$, \ie:
%$$\begin{array}{lcl}
%\lnorm{\cC} \defeq \displaystyle \max_{i\in [1,m]} \{ \lnorm{\cube_i} \} &  & \unorm{\cC} \defeq \displaystyle \max_{i\in[1,m]} \{ \unorm{\cube_i} \}.
%\end{array}$$
%The $l$-norm (respectively $u$-norm) of a counting set $\cSet$ is the smallest $l$-norm (respectively $u$-norm) of a counting constraint representing $\cSet$.
%%that is
%%$$\begin{array}{lcl}
%%\lnorm{\cSet} \defeq \displaystyle \min_{\cSet = \sem{\cC}} \{ \lnorm{\cC} \} &  & \unorm{\cSet} \defeq \displaystyle  \min_{\cSet = \sem{\cC}} \{ \unorm{\cC} \}.
%%\end{array}$$

\subparagraph*{Parameterized Problems.} We define the parameterized versions of the classic problems of reachability, coverability and liveness. 
\begin{itemize}
\item 
\emph{Cube-reachability (coverability):} Given a net $\net$ and cubes $\cube,\cube'$ of $\N$, decide if there are markings $M \in \cube$ and $M' \in \cube'$ such that $M$ is reachable (coverable) from $M'$.
\item
\emph{Cube-liveness:} Given a net $\net$ and a cube $\cube$ of $\N$, decide whether every marking of $\cube$ is live.
Recall that a marking $M_0$ is \emph{live} if for every marking $M$ reachable from $M_0$ and for every transition $t$ of $\net$, some marking reachable from $M$ enables $t$.
\end{itemize}

In~\cite{conf/apn/EsparzaRW19}, we showed that these problems are \PSPACE{}-complete for IO nets. Since a counting set is a finite union of cubes, the problems over counting sets instead of cubes are also \PSPACE{}-complete. We use the Shortening Theorem to prove that the problems are also in \PSPACE{} for \bio{} nets.

We introduce a measure of the size of a cube. The $l$-norm and the $u$-norm of a cube $\cube=(L,U)$ are defined by:
$$\begin{array}{lcl}
\lnorm{\cube} \defeq \displaystyle \sum_{p \in P} L(p) & \quad & \unorm{\cube} \defeq \displaystyle \sum_{\substack{p\in P\\ U(p)<\infty}} \!\!\!\!U(p) \mbox{ (and \( 0\) if \(U(p)=\infty\) for all \(p\))}.
\end{array}$$
The $l$-norm ($u$-norm) of a counting constraint $\cC = \sem{\cube_1,\ldots,\cube_k}$ is the largest $l$-norm ($u$-norm) of a cube in $\cC$.
%, \ie:
%$$\begin{array}{lcl}
%\lnorm{\cC} \defeq \displaystyle \max_{i\in [1,m]} \{ \lnorm{\cube_i} \} &  & \unorm{\cC} \defeq \displaystyle \max_{i\in[1,m]} \{ \unorm{\cube_i} \}.
%\end{array}$$
The $l$-norm ($u$-norm) of a counting set $\cSet$ is the smallest $l$-norm ($u$-norm) of a counting constraint representing $\cSet$. We prove:

%%%%copied from PN20 submission
\begin{restatable}{lemma}{BIOCubePreimage}
\label{lemma:bio-cube-preimage}
The pre-image $\prestar(\cube)$ of a cube $\cube$ in a BIO net with $n$ places is a counting set satisfying $\unorm{\pre^*(\cube)} \leq \placeCount  (\lnorm{\cube} + \unorm{\cube} + \placeCount)$ and $
\lnorm{\pre^*(\cube)} \leq  \placeCount  (\lnorm{\cube}+ \unorm{\cube} +\placeCount)$.
\je{Are both bounds the same??} \cwk{yes}
\end{restatable}

In the proof, we add token-destroying transitions to the net in order to reduce the problem to single-marking pre-image.
%%%%end of copied from PN20 submission
Then we use the token bound from the Shortening Theorem to bound the size of the pre-image of a marking.

%Lemma \ref{lemma:bio-cube-preimage} allows us to prove that 
The cube-parameterized results for IO nets also hold for \bio{} nets. 

\begin{restatable}{theorem}{TheoremBioCube}
The cube-reachability, cube-coverability and cube-liveness problem for \bioLong{} nets are \PSPACE-complete.
\end{restatable}
%%%%end of copied from PN20 submission
 
By Savitch's Theorem, \NPSPACE=\PSPACE, so it is sufficient to provide a nondeterministic algorithm to prove that these problems are in \PSPACE{}.
The algorithm for cube-reachability 
from $\cube'$ to $\cube$ 
guesses a firing sequence step by step,
starting at a marking of size bound by Lemma \ref{lemma:bio-cube-preimage},
guessing each time a marking of size bound by the BIO Shortening Theorem, 
and checking after each step if the reached configuration
is in $\cube$.
The cube-coverability and cube-liveness problems are solved in a similar way.
IO nets are a subclass of \bio{} nets, so the parameterized problems stay \PSPACE-hard for \bio{} nets.

\cwk{here could be a good place for the remark that these results hold also for multi-observation extensions of the models + no source place in BIO extension}
